Predictive Edge Computing with Hard Deadlines

Edge computing is a promising approach for localized data processing for many edge applications and systems including Internet of Things (IoT), where computationally intensive tasks in IoT devices could be divided into sub-tasks and offloaded to other IoT devices, mobile devices, and / or servers at the edge. However, existing solutions on edge computing do not address the full range of challenges, specifically heterogeneity; edge devices are highly heterogeneous and dynamic in nature. In this paper, we develop a predictive edge computing framework with hard deadlines. Our algorithm; PrComp (i) predicts the uncertain dynamics of resources of devices at the edge including energy, computing power, and mobility, and (ii) makes sub-task offloading decisions by taking into account the predicted available resources, as well as the hard deadline constraints of tasks. We evaluate PrComp on a testbed consisting of real Android-based smartphones, and show that it significantly improves energy consumption of edge devices and task completion delay as compared to baselines.

==> evaluation.tex <==

\section{\label{sec:performance} Performance Evaluation}

In this section, we evaluate our online {\em mobility-aware cooperative computation} (MaCC) scheme using a testbed that consists of Android based smartphones. The evaluation results show that our scheme significantly reduces energy and delay as compared to (i) no-cooperation, where device $\eta_0$ processes the tasks by itself, (ii) full offloading, where all the tasks are offloaded from $\eta_0$ to other mobile devices according to a fixed policy. Next, we present testbed setup and results in detail. 

%where each device receives its content from the source without cooperating with other devices,  and (ii) cooperation, where multiple mobile devices cooperate, but the cooperating devices do not do computation and energy control for other devices (mobile devices just receive packets from the source, and relay them to other mobile devices without processing and energy control). Next, we present testbed setup and results in detail. 

\subsection{Setup \& Implementation Details}
{\em Devices:} We implemented a testbed of the setup shown in Fig.~\ref{fig:setup} using real mobile devices, specifically Android 5.1.1 based Nexus 5 smartphones. One of the devices is selected as the task offloading device $\eta_0$, while the other devices are dedicated to process the tasks if they are offloaded. 

{\em Protocol Stack:} We implemented our online MaCC algorithm on top of TCP. This kind of implementation has  advantages as (i) mobile devices do not need rooting, and (ii) our framework and codes could be easily transferred to mobile devices using other operating systems such as iOS.\footnote{We note that we will make our codes and applications publicly available, which we believe will contribute to the research community.} 

{\em Device $\eta_0$:} The task originator device $\eta_0$ is running two applications simultaneously. The first application is playing a pre-stored video. The goal of this application is smoothly playing video after playback starts. The second application is offloading a computationally intensive task to other devices. In terms of such a computationally intensive application, we implemented a text search algorithm, which is explained further next. 

{\em Task:} The text search algorithm in $\eta_0$ should process 200 tasks. Each task contains $40K$ packets, where each packet consists of $500$B. Each task should process all its $40K$ packets to learn if each packet contains a specific text pattern, \eg  ``0123456789''. 

In this setup, $\eta_0$ should either wait for the completion of video playback, or offload the search task to other mobile devices so that video quality is not degraded. 

{\em Devices $\eta_n$:} The task processing device $\eta_n$, $n \neq 0$ receives tasks from $\eta_0$. In particular, $\eta_n$ receives $40K$ packets per task, and searches a specific text pattern in these packets. After completing the search, $\eta_n$ transmits the search results back to $\eta_n$. Note that the search results in this setup are Booleans showing if the string is found in a packet or not. 

{\em Mobility:} In our implementation, we created a simulated mobility in a lab environment. In particular, a device $\eta_n$ exchanges the mobility probability at every 10 sec. This probability is used in our online MaCC algorithm to determine whether to offload tasks or not. Then, the mobile device  creates a random mobility realization, and moves away according to this realization.  

{\em Measuring Delay and Energy Consumption:} The mobile device $\eta_0$ periodically (at every 10 sec) probes other mobile devices to measure the transmission/reception and processing delay and energy consumption. An average of these values over a window of last measurements are calculated and used in our online MaCC algorithm. 

{\em Control Packets:} There are two types of control packets in our implementation. First, mobility, delay, and energy consumption packets are exchanged via D2D connections. As the D2D connections can achieve high transmission rates, the overhead of these control packets are negligible. The second set of control information is needed to localize each mobile device, and create a cooperative group. Ideally, these control packets should be transmitted to a remote server in a cloud, but in our implementation, these control packets are transmitted to (via D2D links) and handled by $\eta_0$. 

{\em D2D Connetions:} All the devices are connected to each other using Wi-Fi Direct connections in our testbed. The task originator device $\eta_0$ is configured as the group owner of the Wi-Fi Direct group. 

{\em Test Environment:} The experiments are conducted in our testbed consisting of Anroid based smartphones in a lab environment, where interference naturally occurs due to multiple Wi-Fi operating devices in the same geographical area. Next, we present our results. 


\begin{table}[t!]
%\vspace{-5pt}
\caption{Task completion time when there is no mobility.}
\centering
\begin{tabular}{  | c | c | }
    \hline  No cooperation & 2243.4  sec \\
    \hline  Full offloading & 2102.8 sec   \\
    \hline  MaCC & 1912 sec \\
    \hline
\end{tabular}
\label{table:completion_time_nomobility}
\vspace{-5pt}
\end{table}

\begin{table}[t!]
%\vspace{-5pt}
\caption{Amount of energy consumption when there is no mobility.}
\centering
\begin{tabular}{  | c | c | c | }
	\hline 				   & $\eta_0$ & $\eta_1$ \\   
    \hline  No cooperation  & 14\%     &  -  \\
    \hline  Full offloading & 15\%     & 12.8\% \\
    \hline  MaCC 		    & 14.6\%   & 9.2\% \\
    \hline
\end{tabular}
\label{table:energy_nomobility}
\vspace{-5pt}
\end{table}

\subsection{Results}
We first consider a setup, consisting of two mobile devices $\eta_0$ and $\eta_1$, where $\eta_0$ plays out a video, and simultaneously offloads tasks (text searching tasks) to $\eta_1$. The initial delay for $\eta_0$ at the start of the experiment is $1600$sec, while it is $0$ for $\eta_1$. The deadline threshold is $\Delta_{thr} = 2500$ sec. In this setup, no cost occurs for transmitting/receiving or processing tasks. Also, there is no mobility in this setup. 

Table~\ref{table:completion_time_nomobility} shows the completion time of the tasks for MaCC as well as the baselines; no cooperation and full offloading. As can be seen, MaCC reduces the completion time as compared to both baselines. No cooperation has higher completion time as compared to full offloading, because $\eta_0$ has higher initial delay. MaCC is better than both baselines, because it takes advantage of both $\eta_0$ and $\eta_1$. We also have a visual results for the same experiment. The captured videos of no cooperation and MaCC are provided in \cite{freezing} and \cite{no_freezing}, respectively, and ready for playout in the links provided by these references for your convenience. As seen in these videos, no cooperation creates a lot of freezing scenes (20\% of playout time), while MaCC provides a smooth video. This experiment demonstrates the importance of computation offloading to improve the quality of other applications, as well as the effectiveness of our algorithm in a real testbed. 

Table~\ref{table:energy_nomobility} shows the amount of consumed energy in terms of percentage of reductions in battery level. As seen, no cooperation has the smallest energy consumption. The reason is that there is no offloading in no cooperation, which saves the data transmission and receiving energy. Yet, although no cooperation is more energy efficient than the other algorithms, its delay performance is quite poor as seen in Table~\ref{table:completion_time_nomobility}, so it is not a viable option in practice. The energy efficiency of MaCC is better than full offloading, because when it does not offload tasks, it saves energy, while full offloading offloads all the tasks. 

\begin{figure}[t!]
\centering
{ {\includegraphics[height = 55mm]{MaCCFigures/mobility_completion_time.eps}} } 
%\vspace{-5pt}
\caption{Completion time when devices are mobile. 0.x/0.y labels in the x-axis demonstrate probabilities that these two devices move away, and get closer, respectively.}
\vspace{-15pt}
\label{fig:mobility_completion_time}
\end{figure}

Now, we consider the mobility scenario. In this setup, there are two mobile devices $\eta_0$ and $\eta_1$. Similar to the previous setup, $\eta_0$ plays a video and offloads a search task to $\eta_1$. The other parameters of the experiment are the same as the previous setup. However, different from the previous setup, $\eta_0$ and $\eta_1$ can move away or get closer over time depending on their mobility patterns. Fig.~\ref{fig:mobility_completion_time} shows the completion time of tasks versus the mobility probability. Note that 0.x/0.y labels in the x-axis of Fig.~\ref{fig:mobility_completion_time} demonstrate probabilities that these two devices move away, and get closer, respectively. As can be seen, no cooperation does not change with mobility, because it does not offload tasks. The completion time of full offloading is small for small mobility probabilities, but it increases exponentially when the mobility increases. This result is expected as full offloading always offloads tasks. On the other hand, the completion time of MaCC is lower than both no cooperation and full offloading. This result shows the significance of mobility-aware computation offloading. 

Fig.~\ref{fig:mobility_energy} shows the energy consumption results at $\eta_0$ and $\eta_1$ for the same setup. As can bee seen no cooperation has the smallest energy consumption level, while our algorithm improves over full offloading. This result shows the importance of joint optimization of delay and energy by taking into account mobility. 

\begin{figure}[t!]
\centering
%\vspace{-5pt}
\subfigure[Energy consumption at $\eta_0$]{ {\includegraphics[height = 55mm]{MaCCFigures/mobility_energy_d0.eps}} } 
\subfigure[Energy consumption at $\eta_1$]{ {\includegraphics[height = 55mm]{MaCCFigures/mobility_energy_d1.eps}} } 
\vspace{-5pt}
\caption{Energy consumption at (a) $\eta_0$, and (b) $\eta_1$, when devices are mobile. 0.x/0.y labels in the x-axis demonstrate probabilities that these two devices move away, and get closer, respectively.
}
\vspace{-15pt}
\label{fig:mobility_energy}
\end{figure}


\section{Basic Studies}
\subsection{Local Processing and Offloading Time}
The time consumption of local processing and offloading is shown in this section. The experiments are performed with old and new nexus 6p phones. Three cases are taken into consideration, local processing with WiFi-Direct on, local processing with WiFi-Direct off and offloading. Ten trials are performed for each case and in each trial, 60 images are processed. 

The local processing with WiFi-Direct on is to use the group owner of a WiFi-Direct group to perform local processing. On the other hand, local processing with WiFi-Direct off is measured on the same phone but the WiFi-Direct group is dismissed. As it is shown in Fig. \ref{fig_1}, for local processing with WiFi-Direct on, there is upward trend of average time per image on both old and new devices. Also, the overall average time consumption is longer than local processing with WiFi-Direct off. The speculated reason for this is that the group owners may spend too much computation resources on maintaining the WiFi-Direct group. We can see if there is similar behavior on Nexus 5 phones by more experiment. Furthermore, new devices process images faster than old devices in the case of offloading and local processing with WiFi-Direct off. The variance is provided in Fig. \ref{fig_2}.

\begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Fig/AverageTime.eps}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{Average time consumption per image.}
\label{fig_1}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Fig/VarAverageTime.eps}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{Variance of time consumption per image.}
\label{fig_2}
\end{figure}

The estimated completion time is calculated by the average completion time of processed images multiplied by the number of images left to be processed. For example, after processing the 10th image, the average comletion time of processed images is calculated by $\sum_{i=1}^{10}t_i/10$, where $t_i$ is the time consumption for processing ith image. After this times 50, which is the number of images left to be processed, the estimated completion time is acquired. 

%The average and variance of the estimated completion time is shown in Fig. \ref{fig_3} and Fig. \ref{fig_4}. 

%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{CompletionTime.eps}
%% where an .eps filename suffix will be assumed under latex, 
%% and a .pdf suffix will be assumed for pdflatex; or what has been declared
%% via \DeclareGraphicsExtensions.
%\caption{Estimated completion time.}
%\label{fig_3}
%\end{figure}

%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{VarCompletionTime.eps}
%% where an .eps filename suffix will be assumed under latex, 
%% and a .pdf suffix will be assumed for pdflatex; or what has been declared
%% via \DeclareGraphicsExtensions.
%\caption{Variance of estimated completion time.}
%\label{fig_4}
%\end{figure}

\subsection{CPU Energy Measurement in Android}
According to the Android source code of class CpuPowerCalculator, the energy consumption of CPU at time t ($E(t)$) is calculated by Equation  (\ref{formula1}), where $T_{ca}(t)$ is the CPU time at time t associated with a particular application, $T_{cs}(t)$ is the CPU time for all the applications in the system at time t, $t_{i,j}(t)$ is the amount of time spent on cluster i of speed j at time t $T_{cs}(t) = \sum_{i = 0}^{i}\sum_{j = 0}^{j}t_{i,j}(t)$, $e_{ij}$ is the average power of cluster i of speed j. 

\begin{equation}\label{formula1}
E(t) = \sum_{i = 0}^{i}\sum_{j = 0}^{j}T_{ca}(t)*t_{i,j}(t)*e_{i,j}/T{cs}(t)
\end{equation} 

CPU time (or process time) is the amount of time for which a CPU was used for processing instructions of a computer program or operating system, as opposed to, for example, waiting for input/output (I/O) operations or entering low-power (idle) mode. The CPU time is measured in clock ticks or seconds. In other words, $T_{ca}(t)$ is the amount of time that CPU has spent to process a particular application. In this case, this particular application is our MaCC app. $T_{ca}(t)$ can be acquired by the method getUserCpuTimeUs. This method takes an input of a integer indicator STATS\_SINCE\_CHARGED or STATS\_SINCE\_UNPLUGGED. For instance, if the STATS\_SINCE\_UNPLUGGED is used, this method will return the amount of time that CPU has spent for this particular application since the device has been unplugged from a power source. $t_{i,j}(t)$ can be obtained by the method getTimeAtCpuSpeed in a similar way. 

In our experiment, at first the device is plugged into a power source. After the device is unplugged, the MaCC applicaton starts and 5 images are processed sequentially and the CPU energy consumption is recorded after each image has been processed. Then it sleeps for 5 seconds for 10 times and the CPU energy is recorded at the end of every 5 seconds. The results are shown in Fig. \ref{fig_5}. As it can be seen that the energy consumption begins to drop after the images are processed and the application goes to sleep. This happens because it uses the ratio of CPU time of the system instead of the application. During the application's sleeping, the system spent a long time running on low speed. However, $T_{ca}(t)$ has little increase as the application is sleeping.

\begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Fig/CPUEnergy.eps}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{CPU energy consumption.}
\label{fig_5}
\end{figure}

There are two solutions for this problem. The first solution is to get the ratio of CPU usage of the particular application instead of the whole system. The corresponding Equation (\ref{formula2}) is given below, where $ta_{i,j}$ is the amount of time spent on cluster i of speed j associated with a particular application.

\begin{equation}\label{formula2}
E(t) = \sum_{i = 0}^{i}\sum_{j = 0}^{j}ta_{i,j}(t)*e_{i,j}
\end{equation} 

 The second solution is to force the devices to use only one cluster at one speed. For example, if cluster i of speed j is used, the energy consumption for a particular application can be calculated by $T_{ca}(t)*e_{i,j}$.
 
 However, these two solutions above are very complicated in terms of implementation. A new method to calculate the energy consumption of a period of time is proposed to overcome this problem. Suppose that the energy consumption between time t and t+$\delta$ (E(t,t+$\delta$)) is desired. E(t,t+$\delta$) can be obtained by 
 
 \begin{equation}\label{formula3}
 \begin{aligned}
 E(t,t+\delta) = \frac{T_{ca}(t+\delta)-T_{ca}(t)}{T_{cs}(t+\delta)-T_{cs}(t)}*\\
 \sum_{i = 0}^{i}\sum_{j = 0}^{j}(t_{i,j}(t+\delta)-t_{i,j}(t))*e_{i,j}
 \end{aligned}
 \end{equation}
 
 At the beginning (t) and ending (t+$\delta$) of processing one image, $T_{ca}(t)$, $T_{ca}(t+\delta)$, $t_{i,j}(t)$ and $t_{i,j}(t+\delta)$ for all i and j can be acquired to calculate the CPU energy consumption more accurately by ruling out the sleeping time.
 
 \subsection{Time Consumption for increased Number of Images }
 In Fig. \ref{fig_1}, the time consumption per image has an upward trend for the case local processing with WiFi-Direct on. Thus, the number of images are increased to 500 from 60 to study whether the time consumption per image will converge to a relatively steady value or not. As shown in Fig. \ref{fig_6}, the time consumption per image will converge after around 150 images. This figure is the average of two trials on both old and new devices.
 
  \begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Fig/Time.eps}
\caption{Time Consumption for increased Number of Images}
\label{fig_6}
\end{figure}
 
 \subsection{Energy consumption}

The average of total energy consumption of CPU and Wi-F versus number of processed images are shown in Fig. \ref{fig_7} and Fig. \ref{fig_8}. There are 10 trials in each plot and the variance are also provided in Fig. \ref{fig_9} and Fig. \ref{fig_10}. The interesting point is that the average Wi-Fi energy consumption for the old devices is slightly higher than the new ones. As the results shown in Fig. \ref{fig_1}, offloading in old devices requires longer time to complete. Therefore, old devices demand Wi-Fi to be on for a longer time thus consume additional energy.

The average energy consumption per image for CPU and Wi-Fi can be found in Fig. \ref{fig_11} and Fig. \ref{fig_12}. The variances are provided by Fig. \ref{fig_13} and Fig. \ref{fig_14}.


 \begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Fig/AveCpu.eps}
\caption{Average CPU Energy Consumption}
\label{fig_7}
\end{figure}
 
 \begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Fig/AveWiFi.eps}
\caption{Average Wi-Fi Energy consumption}
\label{fig_8}
\end{figure} 

% \begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{Fig/VarCpu.eps}
%\caption{Variance of CPU Energy Consumption}
%\label{fig_9}
%\end{figure}
%
% \begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{Fig/VarWifi.eps}
%\caption{Variance of Wi-Fi Energy Consumption}
%\label{fig_10}
%\end{figure}

 \begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Fig/ave_cpu_per.eps}
\caption{Average CPU Energy Consumption per Image}
\label{fig_11}
\end{figure}
 
 \begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Fig/ave_wifi_per.eps}
\caption{Average Wi-Fi Energy consumption per Image}
\label{fig_12}
\end{figure} 

% \begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{Fig/var_cpu_per.eps}
%\caption{Variance of CPU Energy Consumption per Image}
%\label{fig_13}
%\end{figure}
%
% \begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{Fig/var_wifi_per.eps}
%\caption{Variance of Wi-Fi Energy Consumption per Image}
%\label{fig_14}
%\end{figure}
 
 The hardware of the old and new Nexus 6P devices are exactly the same and they both run on Android 6.0.1. The only difference is their Linux kernal version, baseband version and build number.

\subsection{Sleeping Impact on Processing Time and Energy}
Fig. \ref{fig_15} and Fig. \ref{fig_16} demonstrate the energy and time consumption for face detection on two hundred images. For the sleeping case, the application will sleep for 5 second after processing each image. For the non-sleeping case, the application will immediately process next image after each processing. As the number of processed images increasing, non-sleeping case consumes less energy but more time to process one image whereas the sleeping case remains steady in terms of energy and time. 

\begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Fig/cpu_more_images.eps}
\caption{CPU Energy consumption per image for Sleeping and Non-sleeping cases}
\label{fig_15}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Fig/time_per_image_sleep_non_sleep.eps}
\caption{Processing Time per image for Sleeping and Non-sleeping cases}
\label{fig_16}
\end{figure}


\section{Implementation Details}
\subsection{Task}
The task is to sequentially detect the faces in $K$ images ($K$ subtasks) within a period of time (D) while maintaining a smooth playback of a video. After each face is detected on one image, a dot is put between the eyes of that face. There are two options to complete one subtask, local processing and offloading. For local processing, the subtask is executed on the originator's CPU. For offloading, the images are forwarded to one of the available helpers via Wi-Fi direct. The chosen helper will detect the faces using its CPU and send back the results to the originator. As local processing requires a lot of CPU resource, the video playback will experience jitters and freezing scenes. Therefore, local processing has to wait until the video finishes playing, which introduces an initial delay denoted by $w_0$. $w_0$ can be viewed as the remaining playback time of the video. Local processing and offloading one subtask are encapsulated in two separate methods at the originator called "local" and "offload", which are introduced in the following subsections.

\subsection{local method}
The main responsibility of local method is to do face detection on one image using the originator's CPU. The local method is implemented in 4 steps. At the beginning, a time stamp is created to mark the starting time $\tau_s$. Also, the initial energy state ($T_{ca}(\tau_s)$ and $t_{i,j}(\tau_s)$) is recorded. Then the image is decoded to bitmap. After decoding, "quick and easy face detector" will detect faces on the decoded bitmap. Results are then compressed and written to a .png file in the external storage.  Finally, the current time ($\tau_c$) and energy state ($T_{ca}(\tau_c)$ and $t_{i,j}(\tau_c)$). Total Time ($\theta_0$) and energy ($e_0$) consumption is returned by calculating  $\theta_0 = \tau_c-\tau_s$ and $e_0 = E(\tau_s,\tau_c)$ (see Equation(\ref{formula3})). 

%(http://www.anddev.org/quick_and_easy_facedetector_demo-t3856.html)
 
\subsection{offload method}

The offload method is to let a helper detect face(s) on one image and retrieve the results. Same as the local method, $\tau_s$ and ($T_{ca}(\tau_s)$ and $t_{i,j}(\tau_s)$) is recorded at the beginning. The originator initiate the offloading by sending an integer containing the size of the image to be sent. After the helper  receiving an acknowledgment less than 0, the method returns as it indicates that the helper is no longer available. Else if the acknowledgment is larger than 0, the originator sends the image to the helper. Then it waits for an integer indicating the size of the results. If the size is larger than 0, the originator will receive data of exact size and write the data to the external storage. And the time used is denoted by $\theta$. Otherwise if the size is less than 0, the method returns as the subtask has failed and has to be re-scheduled again. For both cases (offloading successful or not), the energy consumptions for the originator ($e_o$ for successful offloading, $\tilde{e}_o$ for failed offloading) and helper ($e_p$ for successful, $\tilde{e}_p$ for failed) are calculated and returned. The helper will send the energy consumption information at the end of every successful subtask to the originator. We assume that the helper will not provide energy consumption to the originator if an offloading is failed. However, we provide test results when the originator can utilize these feedbacks no matter the offloading is successful or not in MaCC new energy model.

\subsection{Helper}
The helper maintains two thread. One thread is the mobility thread discussed in the subsections bellow. Another thread is called the processor thread introduced after mobility thread. It is to communicate with the originator and process the images.These two threads run in parallel. To simplify the scenario, we simulated the mobility in mobility thread following a mobile model (pattern).

\subsubsection{Mobility Model}
\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/mo1.pdf}
	% where an .eps filename suffix will be assumed under latex, 
	% and a .pdf suffix will be assumed for pdflatex; or what has been declared
	% via \DeclareGraphicsExtensions.
	\caption{Markov Chain of the Mobility Model}
	\label{fig_23}
\end{figure}

The helpers are mobile. That means the helpers are not always available. The helpers have two states, either inside the originator's communication range (True) or outside {False}. The simulation of mobility is implemented in a 5-second or 10-second slotted fashion. Let $t_n$ (n = 0,1,2...) denote the beginning of the nth slot. When the current state $C(t_n)$ is True, there is a probability of leaving the originator ($P_l$) at $t_{n+1}$. Otherwise when the helper is outside the range of originator, there is a probability for the helper to return to the originator ($P_c$). Furthermore, the state of the helpers is fixed during one slot ($C(t_n) = C(t_n+\delta)$ for $0\leq\delta\leq 10$).  We set $C(t_0)$ to be True representing that initially all the helpers are in the range. The transition between two states forms a Markov chain shown in Fig. \ref{fig_1}.  

\subsubsection{Mobility Thread}
Mobility is simulated in an independent thread. The states of the helper is represented by a boolean variable. During the execution of each task, the helper will check this boolean and act accordingly. The randomness is introduced by a uniformly distributed random number (u) between 0 and 1 generated at the beginning of each slot. When the current state is True and u is less than $P_l$ the state will change to False. On the other hand, if the state is currently False and u is less than $P_c$, the state will switch to True. The detailed implementation is illustrated in Algorithm \ref{alg1}.

\subsubsection{Processor Thread}
Processor thread needs to correspond to the offload method at the originator. In each subtask, there are three steps: receiving original data (image), processing the data and sending back results. First it receives an integer indicating the size of the image from the originator. It represents the beginning of step 1. The helper then receive the image. After receiving the image, step 2 begins. The image are further decoded to a bitmap. By using "quick and easy face detector", faces are detected on the bitmap and converted the results to a byte stream to be sent through the socket. After processing, step 3 starts. Finally, the byte stream is sent to the originator. Fig. \ref{fig_24} provides the flow chart of a helper executing one subtask that is offloaded by the originator. If the helper's state is false at the beginning of each step, the helper will notify the originator that the current subtask has failed and the rest steps are not continued. Naturally, the originator has to reschedule this task. If one subtask is successfully completed, the energy consumption information will be sent to the originator.
\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/processor.pdf}
	\caption{Helper's Flow Chart}
	\label{fig_24}
\end{figure}

%\begin{algorithm}
%	\SetAlgoLined
%	% \KwData{this text}
%	% \KwResult{how to write algorithm with \LaTeX2e }
%	% initialization\;
%	\caption{Mobility Implementation of MaCC}
%	boolean c = true\;
%	\While{task not completed}{
%		%  read current\;
%		u is uniformly chosen between 0 and 1.\\
%		\If{c=true(processing device is in the range of originator)}{
%			\If{u $ < P_l$}{
%				c = false;
%			}
%		}
%		\Else{
%			\If{u $< P_c$}{
%				c = true;
%			}
%		}
%		Thread sleeps for 5 or 10 seconds.
%	}
%	\label{alg1}
%\end{algorithm}



\subsection{No Cooperation Implementation}
In this case, the originator does not cooperate with other processors (or helpers). Every task is done locally. As the originator has to finish playing a video first, the processing starts after the video playback. The local method is repeatedly executed N times as there are N subtasks. After one subtask is completed, the next subtask starts immediately until all the subtasks are completed. 

\subsection{Full Offloading Implementation}
For the full offloading case, the originator will not process any image locally. All the subtasks are offloaded to the helpers. If there are multiple helpers, the subtasks are scheduled in a round-robin fashion. The originator maintains a list of all the N helpers ($h_1$, $h_2$,..., $h_N$ ). Let's suppose one subtask is scheduled to $h_n$ and $h_n$ successfully completed this subtask. Next subtask will be scheduled to $h_{n+1}$ if $h_{n+1}$ is within the system (available). Otherwise, it keeps searching ($h_{n+2}$, $h_{n+3}$,$h_{n+4}$, ...) until an available helper is found. (If $h_N$ is reached, originator will go back to $h_1$ next time.) Then the subtask is offloaded to that helper. If $h_n$ (n = 1,2,...N) failed to complete the current subtask, the originator also will search for next available helper immediately after the failure and offloaded the current task to that helper. If all the helpers are gone, it waits (sleeps) for 0.5 second then checks from the first helper. Note that when one of the helpers is processing, other helpers and the originator are resting as the execution is blocked by I/O. 

\subsection{MaCC Implementation}
MaCC can utilize both offloading and local processing. Local processing can be viewed as helper 0 ($h_0$), which is always available as long as the video is not playing. By looking at the time and energy consumption for each helper to complete one subtask, MaCC can schedule each subtask to the most appropriate helper. The implement of MaCC consists three phases. The first phase is checking availability. If the helper is out of the system or the video is still playing for $h_0$, originator will move on to the next helper. Otherwise if the helper is available, the originator should move to phase 2 and determine whether scheduling the current subtask to the specific helper can meet the deadline requirement or not. The estimated completion time of helper n at subtask $k$ ($k = 0,...,K$) can be given as 

\begin{equation}\label{formula4}
T_{n,k} = w_n+t_n+t_0*P_n+((t_0+t_n)/2*(1-P_n)+t_0*P_n)*(K-k)
\end{equation}

where $w_n$ is the initial delay of $h_n$. $t_n$ (n = 0,1,..N) is the average time needed 
for $h_n$ to complete one subtask. $t_n$ is calculated by $\sum_{i_n=1}^{M_n}\theta_n^{i_n}/{M_n}$, where $\theta_n^{i_n}$ is the time used if the $i_n^{th}$ subtask is successfully offloaded to $h_n$. $M_n$ is the number of subtasks successfully completed by $h_n$. Note that $k = \sum_{n=0}^NM_n$. $P_n$ is the probability of leaving for $h_n$.

If $T_{n,k}$ is less than the remaining time to complete the whole task, the originator goes to phase 3, energy estimation. The energy consumption for helper n $h_n$ is estimated by 3 different models discussed in the following subsections.

\subsubsection{MaCC Ordinary}

\begin{equation}\label{formula5}
E_n(k) = \epsilon_n(k)+\epsilon_0(k)*P_n
\end{equation}

where $\epsilon_n(k)$ ($n = 0,1,2...N$)is the average energy consumption for $h_n$ to successfully completing one subtask. $\epsilon_n(k)$ is calculated by
$$\epsilon_n(k) = \sum_{i_n=1}^{M_n(k)}(e_{o,n}^{i_n}+e_{p,n}^{i_n})/M_n(k)$$
where $e_{o,n}^{i_n}$ and $e_{p,n}^{i_n}$ is the energy consumption for the originator and helper n $h_n$ to successfully complete subtask $i_n$ respectively. $M_n(k)$ is also the number of successful subtasks completed by $h_n$ when the current subtask is k. $k = \sum_{n=0}^NM_n(k)$.

Among all the helpers that can meet the deadline, schedule the subtask to the one that consumes the least energy ($E_n(k)$).

\subsubsection{MaCC New Energy Estimation Model}
To estimate the energy consumption for each helper n, the MaCC requires the helper's probability of leaving ($P_n$), which is not always available in reality. The MaCC New Energy Estimation model is proposed to address this issue. When the Originator tries to offload a task to one of the helpers, there is a chance that the task will fail due to mobility. If the helper has high mobility, most likely it will "waste" the time and energy not successfully completing a task. Therefore, the essential idea is to calculate the average energy consumption per successful task for helper n (n=0,1,2...N, helper 0 is local processing) and use the average value to schedule tasks. Note that there are N helpers in the system. The calculation is given by

\begin{equation}\label{formula6}
E_n(k) = s_n(k)/M_n(k)
\end{equation}
where $s_n(k)$ is the total energy consumption (including wasted energy with or without the helpers information) spent on helper n and $M_n(k)$ is the number of successfully completed tasks by helper n. $s_n(k)$ is calculated by 

$$s_n(k) = \sum_{i_n=1}^{\tilde{M}_n(k)}(\tilde{e}_{o,n}^{i_n}+\tilde{e}_{p,n}^{i_n})+\sum_{i_n=1}^{M_n(k)}(e_{o,n}^{i_n}+e_{p,n}^{i_n})$$

where $\tilde{M}_n(k)$ is the total number of failed subtasks by $h_n$. $\tilde{e}_{o,n}^{i_n}$ and $\tilde{e}_{p,n}^{i_n}$ are the energy consumption for the originator and helper n respectively when the $i_n^th$ failed subtask.

For real-world scenarios, 
$$s_n(k) = \sum_{i_n=1}^{\tilde{M}_n(k)}\tilde{e}_{o,n}^{i_n}+\sum_{i_n=1}^{M_n(k)}(e_{o,n}^{i_n}+e_{p,n}^{i_n})$$

as $\tilde{e}_{p,n}^{i_n}$ is most probability unavailable if helper has left the communication range of the originator.

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/Drawing1.pdf}
	\caption{Implementation of New Model}
	\label{fig_22}
\end{figure}
In order to achieve the model described above, a double array of size N+1 (E) and a counter (integer) array of Size N+1 (C) are created. Suppose N is the number of helpers. The indexes of the arrays correspond to each helper. Helper 0 is local processing. E(n) is the total energy consumption for helper n (n = 0,1,...N). C(n) indicates the number of tasks that helper n (n = 0,1,...N) has successfully completed. Let us suppose that the originator decides to offload one task to helper n. When the originator receives the results from the helper, the energy consumption is added to E(n) whether the task is successfully completed or not. However, if the task is successfully completed, the counter C(n) will be increased by 1. On the next iteration, among all available helpers, the helper with minimum value of  $E_m(n)$ = E(n)/C(n) is chosen to complete the current task. Fig. \ref{fig_22} illustrates this model.

\subsubsection{MaCC Newest Energy Estimation Model}
Since the CPU energy consumption of the Nexus 5 is fluctuating dramatically, the MaCC Newest Energy Estimation model is proposed to better reflect the changes of energy consumption. It uses the weighted average to estimate the energy consumption. It is given by 

\begin{equation}\label{formula7}
E_n(k) = \gamma_n(k)+\gamma_0(k)*P_n
\end{equation}
where $\gamma_n(k)$ is given by 
$$\gamma_n(k) = 0.8*(e_{o,n}^k+e_{p,n}^k)+0.2*\gamma_n(k-1)$$ 
if the last successful subtask is completed by $h_n$. $e_{o,n}^k$ and $e_{p,n}^k$ is the energy consumption for the originator and helper n respectively. For other helpers, 
$$\gamma_n(k) = \gamma_n(k-1)$$

\section{Parallel Processing}
In the previous section, the subtasks are executed serially as sub-task n can only start when sub-task n-1 is completed. In this section we look at the case where sub-tasks can be completed at the same time. A new algorithm is proposed to schedule subtasks to let all the subtasks be completed by a certain deadline while maintaining the lowest energy consumption. In order to offload multiple subtasks simultaneously, multi-threading is needed. Traditional threads will not have return values so callable interfaces are implemented instead of runnable. First of all, the energy consumption for all the helpers (including local processing) are estimated (see MaCC Implementation section) and sorted. Starting from the one with the least energy consumption, execute the offloading by submit the callable to the thread pool if the helper (or local processing) is available. Then the scheduler estimates how many subtasks can this helper (or local processing) complete before the deadline. If this number is less than the remaining number of subtasks, it means the estimated completion time failed to meet the time constraint. Therefore, the option with the second least energy consumption is chosen. The procedure will repeat until the deadline is met.
After the scheduler goes through all the helpers, the originator will start to retrieve results from all the helpers and local processing with a timeout (10 seconds).

%\begin{algorithm}
%	\SetAlgoLined
%	\caption{Baseline Parallel Scheduling Algorithm}
%	\While{task not completed}{
%		\For{All the helpers including originator itself}{
%			\If{processing device is available}{
%				submit to thread pool
%			}
%			\Else{
%				test availability
%			}
%		}
%		\For{all the threads in the thread pool}{
%			retrieve results
%		}
%	}
%	\label{alg2}
%\end{algorithm} 

The baseline scheduling algorithm will try to utilize every available helper(s) (including originator itself). The algorithm is illustrate in algorithm \ref{alg3}. At each scheduling iteration, the originator will find all available helpers and offload the task to them. If local processing is also available, the originator itself will also execute one subtask.

%\begin{algorithm}
%	\SetAlgoLined
%	\caption{Baseline Parallel Scheduling Algorithm}
%	\While{task not completed}{
%		\For{All the helpers including originator itself}{
%			\If{processing device is available}{
%				submit to thread pool
%			}
%			\Else{
%				test availability
%			}
%		}
%		\For{all the threads in the thread pool}{
%			retrieve results
%		}
%	}
%	\label{alg3}
%\end{algorithm}

\section{Evaluation}

We tested the performance of various versions of MaCC comparing to full-offloading and local processing. Firstly, we demonstrated and analyzed the performance of MaCC when the tasks are serial then we expanded our view to the parallel case.

\subsection{Performance with Mobility against Number of Helpers}
Fig. \ref{fig_25} and Fig. \ref{fig_26} demonstrates the completion time and energy consumption against the number of helpers. This figure is generated by 16 trials for each case. The time step for mobility is 10 seconds, with one helper 0.3/0.5 and the rest 0.9/0.9. In each trial 60 images are processed and the deadline for MaCC is 600 seconds. The minimum and maximum value of each data is also provided by the difference bar. 
We can see that the completion time does not increment with the increasing number of helpers although the number of failed jobs are increasing in the full offloading case. The reason is that when the number of helpers are small (1 or 2), the main delay factor is the lack of available helper. If there is no available helper, the originator will have to wait until one comes back. But with more helpers (4 or 5), the time is wasted on unsuccessful offloading. However, waiting costs less energy comparing to unsuccessful offloading. Therefore, we can see the energy consumption increases with the increasing number of helpers. Fig. \ref{fig_27} and Fig. \ref{fig_28} is another 6 trials on the full offloading for the number of failed tasks, completion time. As shown in the figures, MaCC can meet the deadline while saving energy comparing to local processing and full offloading. The energy consumption for different energy estimation models behaves similarly. MaCC Ordinary is using average based algorithm to make scheduling decisions, which can not reflect the fluctuation of energy consumption in local processing so the energy consumption is a little higher than the other two schemes. The energy consumption of MaCC new model slightly increases when the number of helpers increases since it requires a couple of more iterations to converge to the optimal solution. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/time_vs_num_helper_10sec_03050909}
	\caption{Completion Time vs Number of Helpers when the time step is 10 seconds}
	\label{fig_25}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/energy_vs_num_helper_10sec_03050909}
	\caption{Energy Consumption vs Number of Helpers when the time step is 10 seconds}
	\label{fig_26}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/FailedJobsForOffload}
	\caption{Number of Failed jobs for offload when time step is 10 seconds.}
	\label{fig_27}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/Completiontimeoffload}
	\caption{Completion time for full offloading}
	\label{fig_28}
\end{figure}

Fig. \ref{fig_29} and Fig. \ref{fig_30} illustrate the performance of MaCC comparing to local processing and full offloading when the mobility time step is 5 instead of 10 seconds. In this case, the helpers are more mobile. Therefore, the chances of having failed jobs increases. For full offloading, the completion time and energy consumption both increase with more number of helpers. The newest model remains relatively steady as it can adapt the changes in the local processing and it does not require collecting initial energy information from the helpers as the new energy model does. The more realistic new energy model consumes more energy when the number of helpers increases because the failed tasks provide less information so it takes more iterations for the originator to find the less mobile helper.

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/5secTime}
	\caption{Completion time when the time-step is 5 seconds }
	\label{fig_29}
\end{figure}
\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/5secEnergy}
	\caption{Energy consumption when the time-step is 5 seconds }
	\label{fig_30}
\end{figure}

\subsection{Performance with Different Helpers and Mobility Pattern}
Table \ref{table_1}, \ref{table_2} demonstrate the completion time and energy consumption when there are two helpers, one Nexus 5 and one Nexus 6P. Nexus 6P has more powerful CPU so it took less time and energy to complete one task.
The MaCC newest can schedule the task in a efficient way to save completion time and energy comparing to No cooperation and Full offloading as full offloading treats helpers with different hardware configurations the same.

%Table \ref{table_3}, \ref{table_4}

\begin{table}[!t]
	\renewcommand{\arraystretch}{1.3}
	\caption{Completion Time One Helper Nexus 5 with Mobility 0.3/0.5 and No mobility}
	\label{table_1}
	\centering
	\begin{tabular}{|c|c|c|c|}
		\hline
		& No cooperation & Full Offloading & MaCC Newest\\
		\hline
		5 sec & 674.1425 s & 629.7340 s & 530.7090 s \\
		\hline
		10 sec & 674.1425 s & 592.9850 s & 506.5080 s \\
		\hline
		No Mobility & 674.1425 s & 419.6430 s & 366.2740 s\\
		\hline
	\end{tabular}
\end{table}
\begin{table}[!t]
	\renewcommand{\arraystretch}{1.3}
	\caption{Energy Consumption One Helper Nexus 5 with Mobility 0.3/0.5 and No mobility}
	\label{table_2}
	\centering
	\begin{tabular}{|c|c|c|c|}
		\hline
		& No cooperation & Full Offloading & MaCC Newest\\
		\hline
		5 sec & 32.1214 mAh & 33.7147 mAh & 29.7604 mAh \\
		\hline
		10 sec & 32.1214 mAh & 33.6211 mAh & 28.2015 mAh \\
		\hline
		No Mobility & 32.1214 mAh & 24.8485 mAh & 21.0540 mAh\\
		\hline
	\end{tabular}
\end{table}

\begin{table}[!t]
	\renewcommand{\arraystretch}{1.3}
	\caption{Completion Time Both Helpers Nexus 6P with Mobility 0.3/0.5 and No mobility}
	\label{table_3}
	\centering
	\begin{tabular}{|c|c|c|c|}
		\hline
		& No cooperation & Full Offloading & MaCC Newest\\
		\hline
		5 sec & 674.1425 s & 511.5530 s & 518.9540 s \\
		\hline
		10 sec & 674.1425 s & 477.4070 s & 463.7470 s \\
		\hline
		No Mobility & 674.1425 s & 340.9700 s & 337.5610 s\\
		\hline
	\end{tabular}
\end{table}

\begin{table}[!t]
	\renewcommand{\arraystretch}{1.3}
	\caption{Energy Consumption Both Helpers Nexus 6P with Mobility 0.3/0.5 and No mobility}
	\label{table_4}
	\centering
	\begin{tabular}{|c|c|c|c|}
		\hline
		& No cooperation & Full Offloading & MaCC Newest\\
		\hline
		5 sec & 32.1214 mAh & 27.8786 mAh & 28.2377 mAh \\
		\hline
		10 sec & 32.1214 mAh & 24.1425 mAh & 25.4356 mAh \\
		\hline
		No Mobility & 32.1214 mAh & 20.6334 mAh & 21.0044 mAh\\
		\hline
	\end{tabular}
\end{table}

\subsection{Parallel Performance Evaluation}

The performance of the proposed algorithm and baseline algorithm are shown in Fig. \ref{fig_para_time} to Fig. \ref{fig_para_dde}. The experiments are to complete 60 subtasks (face detection) with 145 seconds initial delay for local processing. The originator is a Nexus 5 and the helpers are all Nexus 6Ps with more powerful and efficient CPUs. The "newest" energy estimation mechanism is used in these experiments for MaCC Parallel. In Fig. \ref{fig_para_time} and Fig. \ref{fig_para_energy}, the deadline is 500 seconds and the completion time and energy consumption against the number of helpers are given. The first helper is less mobile (0.3/0.5) and if there are more than one helper, the other helper(s) is/are with mobility (0.9/0.9).  With the increasing number of helpers, the completion time for the baseline decreases but the energy consumption increases. This is because the baseline offloads indistinguishably to all available helpers despite that they are highly movable and more likely to waste energy. With the increased number of helpers, the completion time decreases since there are more tasks done simultaneously. Whereas the MaCC Parallel can avoid the helpers with high mobility and offloads to the first helper or local processing since the deadline is not tight. Similar situation also applies when the rest helper is less mobile (0.6/0.9 instead of 0.9/0.9) as illustrated in Fig. \ref{fig_para_time06} and Fig. \ref{fig_para_energy06}. The only difference is that when the helpers are less likely to move during a execution, the overall completion time and energy consumption decreases.

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/para_time}
	\caption{Completion time of parallel processing when one of the helper is 0.3/0.5 others 0.9/0.9 with time step 5 seconds.}
	\label{fig_para_time}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/para_energy}
	\caption{Energy consumption of parallel processing when one of the helper is 0.3/0.5 others 0.9/0.9 with time step 5 seconds.}
	\label{fig_para_energy}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/para_time_06}
	\caption{Completion time of parallel processing when one of the helper is 0.3/0.5 others 0.6/0.9 with time step 5 seconds.}
	\label{fig_para_time06}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/para_energy_06}
	\caption{Energy consumption of parallel processing when one of the helper is 0.3/0.5 others 0.6/0.9 with time step 5 seconds.}
	\label{fig_para_energy06}
\end{figure}

 Fig. \ref{fig_para_ddt} and Fig. \ref{fig_para_dde} demonstrate that MaCC parallel can adapt with different deadlines (from 200 to 500 seconds) and save energy when the deadline is not tight. This is because MaCC parallel can exclude helpers that cost more energy when the energy-efficient helpers can meet the deadline. When the deadline is tight, the MaCC behaves like the baseline to utilize all the resources that is available. The performance of the baseline is independent of deadline since it does not take into consideration of the deadline when it makes decisions. The energy consumption of MaCC Parallel stops decreasing when the deadline is expanded to 400 seconds. At that point, only local processing and the helper less mobile (0.3/0.5) are involved. The average energy consumption to complete one subtask is similar for these two approaches. For 400-second deadline, these two approaches are selected simultaneously more often to save completion time. For 450-second and longer deadlines, the originator will only select the one that cost least energy. However, the second least energy consuming one is very close to the least energy consumer. Therefore the energy consumption is very close for the deadlines over 400 seconds. ARC on the other hand, is trying to offload all subtasks to every available helper since it decides offloading will benefit for reducing the local footprint. The total energy consumption for ARC and opportunistic approach is similar. However, when we look at the energy consumption at the originator alone, ARC costs 0.99 mAh and opportunistic costs 2.27 mAh. In other words, ARC can reduce local footprint and fulfill its objective. Later the results of originator's energy consumption for shorter initial delay will show more significant difference for ARC and opportunistic.
 
\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/diffdeadt}
	\caption{Completion time of parallel processing when one of the helper is 0.3/0.5 others 0.6/0.9 with time step 5 seconds. Total 5 helpers different deadline.}
	\label{fig_para_ddt}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/diffdeade}
	\caption{Energy consumption of parallel processing when one of the helper is 0.3/0.5 others 0.6/0.9 with time step 5 seconds. Total 5 helpers different deadline.}
	\label{fig_para_dde}
\end{figure}
%dfafda , Fig. \ref{fig_para_energy}, Fig. \ref{fig_para_time06}, Fig. \ref{fig_para_energy06}, Fig. \ref{fig_para_ddt} and 

Table \ref{table_5} and Table \ref{table_6} shows the performance of MaCC Parallel and the baseline algorithm in terms of completion time and energy consumption when the helpers are heterogeneous in processing speed and energy consumption. In this case, we uses one Nexus 5 (2013) and one Nexus 6P (2015) with the same mobility patterns as two helpers. Nexus 6P has more powerful and efficient CPUs. Thus, it cost less energy and time to complete one subtask and it is more preferable than Nexus 5 if the deadline is not tight. The result shows that MaCC Parallel will save energy by choosing the 6Ps more often comparing to the baseline while meeting the deadline.

\begin{table}[!t]
	\renewcommand{\arraystretch}{1.3}
	\caption{Completion Time One Helper Nexus 6P One Helper Nexus 5 with Mobility 0.3/0.5 and No mobility 500 seconds deadline}
	\label{table_5}
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		& No cooperation & Base Line & ARC & MaCC Newest\\
		\hline
		5 sec step& 674.14 s & 259.12 s & 356.82 s & 468.52 s \\
		\hline
		No Mobility & 674.14 s & 219.45 s & 253.73 s & 344.03 s\\
		\hline
	\end{tabular}
\end{table}

\begin{table}[!t]
	\renewcommand{\arraystretch}{1.3}
	\caption{Energy Consumption One Helper Nexus 6P One Helper Nexus 5 with Mobility 0.3/0.5 and No mobility 500 seconds deadline}
	\label{table_6}
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		& No cooperation & Base Line & ARC & MaCC Newest\\
		\hline
		5 sec step& 32.12 mAh & 33.24 mAh & 34.94 mAh& 27.85 mAh \\
		\hline
		No Mobility & 32.12 mAh & 25.53 mAh & 24.09 mAh & 20.28 mAh\\
		\hline
	\end{tabular}
\end{table}

\subsubsection{Shorter initial delay}

Fig. \ref{fig_para_time20} and Fig. \ref{fig_para_energy20} shows the completion time and total energy consumption for MaCC parallel, ARC and opportunistic when the initial delay is 20 seconds instead of 145 seconds. These two figures have similar patterns with Fig. \ref{fig_para_ddt} and Fig. \ref{fig_para_dde}. Fig. \ref{fig_para_originator} demonstrates the energy consumption at the originator. For MaCC parallel, the energy consumption increases when the deadline increases from 200 to 350. When the deadline is tight, more highly mobile helpers are involved simultaneously to meet the deadline. Hence, less subtasks are done by the originator itself. The average total energy consumption to complete a subtask by a high mobility helper is more than local processing. When the deadline becomes looser, originator offloads less tasks to high mobile helpers in order to save total energy consumption. Thus, more and more subtasks are executed locally and more energy is consumed at originator. On the other hand, when the deadline becomes even less constrained from 350 to 500 seconds, less subtasks are done by the originator and more subtasks are completed by the helper that is less mobile. Since less expected energy consumption to complete one subtask is needed for the helper that has low mobility than local processing. Offloading to the low mobility helper alone can meet the longer deadlines for most of the time. Therefore, the originator does not have to process many subtasks itself. Then energy consumption drops.

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/time20}
	\caption{Completion time of parallel processing when one of the helper is 0.3/0.5 others 0.6/0.9 with time step 5 seconds.The initial delay is 20 seconds.}
	\label{fig_para_time20}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/energy20}
	\caption{Total energy consumption of parallel processing when one of the helper is 0.3/0.5 others 0.6/0.9 with time step 5 seconds.The initial delay is 20 seconds.}
	\label{fig_para_energy20}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{Fig/originator}
	\caption{Originator's energy consumption of parallel processing when one of the helper is 0.3/0.5 others 0.6/0.9 with time step 5 seconds.The initial delay is 20 seconds.}
	\label{fig_para_originator}
\end{figure}


